The Informal Labor of Content Creators: Situating Xiaohongshu's Key Opinion Consumers in Relationships to Marketers, Consumer Brands, and the Platform

This paper critically examines flexible content creation conducted by Key Opinion Consumers (KOCs) on a prominent social media and e-commerce platform in China, Xiaohongshu (RED). Drawing on nine-month ethnographic work conducted online, we find that the production of the KOC role on RED is predicated on the interactions and negotiations among multiple stakeholders -- content creators, marketers, consumer brands (corporations), and the platform. KOCs are instrumental in RED influencer marketing tactics and amplify the mundane and daily life content popular on the platform. They navigate the dynamics in the triangulated relations with other stakeholders in order to secure economic opportunities for producing advertorial content, and yet, the labor involved in producing such content is deliberately obscured to make it appear as spontaneous, ordinary user posts for the sake of marketing campaigns. Meanwhile, the commercial value of their work is often underestimated and overshadowed in corporate paperwork, platform technological mechanisms, and business models, resulting in and reinforcing inadequate recognition and compensation of KOCs. We propose the concept of ``informal labor'' to offer a new lens to understand content creation labor that is indispensable yet unrecognized by the social media industry. We advocate for a contextualized and nuanced examination of how labor is valued and compensated and urge for better protections and working conditions for informal laborers like KOCs.

==> commands.tex <==
%%%%%%% comments %%%%%%%%%%%%%%%
\usepackage{soul}
\usepackage{subcaption}
\usepackage{multirow}
\usepackage{csquotes}

%%%%%%% general comments & bugmarks %%%%%%%%%
\newcommand{\Comment}[1]{}
\newcommand{\NOTE}[1]{\marginpar{\em {#1}}}
\newcommand{\bug}
    {\mbox{\rule{2mm}{2mm}}}
\newcommand{\Bug}[1]
    {\bug \footnote{BUG: {#1}}}
%\newcommand{\chm}[1]{\textcolor{red}{#1}}
\newcommand{\chm}[1]{#1}

%%%%%%% drawing and figures %%%%%%%%%%%%%%%
\usepackage{graphicx}
\usepackage{enumitem}
\setlist[description]{leftmargin=2\parindent,labelindent=2\parindent,rightmargin=2\parindent}

%%%%%%% bullets %%%%%%%%%%%%%%%
\setlist[itemize]{leftmargin=*}
\setlist[enumerate]{leftmargin=*}
\newcommand{\myquote}[1]{
     {{``}\emph{#1}{''}}
}

%%%%%%%% Other stuff
%\usepackage{draftwatermark}
%\SetWatermarkText{Do Not Distribute}
%\SetWatermarkLightness{0.9}
%\SetWatermarkScale{0.5}

==> scratch/Positionality.tex <==
%\section{Positionality}


%The research team includes two graduate students based in an educational institution in the United States. The first author, as a non-Chinese speaker, certain interactions led to ``communicatively ambiguous social encounters in the field'' \cite[p.10]{abu1990can}. As this piece investigates a phenomenon in a Chinese context, this language barrier foreclosed certain engagement opportunities. Many translation applications and sites were utilized to find one suitable for translation. In this case, a constant dialogue was kept open between the first author and the second author to support the investigation. As a non-Chinese individual, I acknowledge the failure of some U.S.-based inquiries into China that position the U.S. researcher as a knower/representer and the Chinese ``subjects'' into knowns/representeds \cite{abu1990can}. It is the first author's hope that this work circumvents this and lets Chinese citizens speak for themselves. 

%The second author follows the feminist sensibilities to conduct ethnographic work with a sense of reciprocity \cite{leavy2018contemporary}. The participant observation on various social media platforms happened on a daily basis. By using comments and private messages, the second author spread information to help people who were caught in medical resources during the sudden zero-COVID policy change and provided emotional and material to support those who would open up to tell how their everyday life in precarity. Second, as a Chinese citizen overseas, the second author's investigation of Paxlovid was also intertwined with her personal experiences of caring for her family and friends in China. Writing the ethnographic vignettes with reflexivity \cite{behar2022vulnerable}, the second author constantly found restlessness that she felt when searching for Paxlovid. It informed the second author to notice the emotions permeating social media postings and personal narrations. However, in the past three years, amid the global pandemic and geopolitical tension with the U.S., the CCP has been portraying itself as capable of protecting its citizens and reaching zero-COVID. The second author noticed negative and personal emotions\cite{lin2021techniques}--insecurity, uneasiness, anxiety, nervousness, sensitiveness, sadness, fear, which led to individualized practices of searching for Paxlovid. Lastly, the second author pushes against the trend of studying China by extracting ``big data'' from social media platforms \cite{wang2021doing, chen2023china} and writes on people's lived experiences observed in her daily immersion in social media platforms and interaction with people.


==> scratch/scratch-0706-draft.tex <==
\section{abstract}

%It highlights the socio-political and economic dynamics shaping young Chinese career choices and their strategies to navigate the employment landscape in a post-pandemic era. 

%In early December 2022, China's zero-COVID policy came to an end. For Chinese citizens, an imaginary of safety predicated on collective action and state care was replaced with a general focus on individualized responsibility for maintaining one's health. This expedited policy reversal had the unintended effect of infecting around 80\% of China’s population in one month, leading to a period of confusion, anxiety, and infection. One way of obtaining safety in a precarious time was to acquire medical resources. Through an online ethnographic investigation, we trace the acquisition of Paxlovid, an antiviral medication that had its distribution within China complicated by geopolitical tension and supply issues. By attending to the precarity of Chinese citizens at home and abroad, we show how Paxlovid was desired in both the present tense for the presently ill and in the future tense as an anticipatory form of safety. We use the analytical lens of anticipation work to unpack individual, collective, and state anticipatory practices. In doing so, we highlight moments of friction between and among various actors to argue that attending to affect, precarity, and moments of conflict is critical to understanding the complexities of collaborative work. 


%After three-year long China's zero-COVID policy, this policy was unceremoniously rescinded. An imaginary of safety predicated on collective action and state care was replaced with a general focus on individualized responsibility for maintaining one's health. This expedited policy reversal had the unintended effect of infecting around 80\% of China’s population in one month, leading to a period of confusion, anxiety, and infection. For Chinese citizens, one way of obtaining safety in a precarious time was to acquire medical resources. Here, we trace the acquisition of Paxlovid, an antiviral medication that had its distribution within China complicated by geopolitical tension and issues of supply. By attending to the precarity of Chinese citizens at home and abroad, we show how Paxlovid was desired in both the present tense for the currently ill and in the future tense as an anticipatory form of safety. We use the analytical lens of anticipation work to unpack individual, collective, and state anticipatory practices. In doing so, we highlight moments of friction between and among various actors to argue that attending to affect, precarity, and moments of conflict is critical to understanding the complexities of collaborative work. 


%This work sheds light on the individualized practices xx that in the political processes in the time of geopolitical tension. 


%We argue that attending to affective and material precarity at a small scale is
%critical to understanding the complexities of collaborative work

%We argue that attending to affective and material precarity at a small scale is critical to understanding the complexities of collaborative work.

%We argue that a sociotechnical state imaginary where the state is able to be free from COVID cases gave way to an unfolding crisis in which, precarious affective and material experiences of individuals motivate them to search for a future of hope through the turmoil of the present. This work shed light on the individualized practices xx that in the political processes in the time of geopolitical tension. 


\section{introduction}
% 通过灵活就业，年轻人可以找到工作的方式，意义，价值
% situate our paper in gig work -- 现在我们观察到的是一种gig work
% \hy{TKTK 年轻人对于工作和生活的焦虑}


% By navigating and adapting to these flexible employment structures, they are not only contributing to the economy but also reshaping their roles and identities within it. This dynamic reflects a complex interplay between individual agency, state policies, and economic forces, highlighting the transformative potential of flexible employment in the modern Chinese context.
% In this paper, we aim to explore how platforms facilitate seemingly flexible employment by providing "side hustle" opportunities for well-educated young urbanists in the platform economy. By focusing on the infrastructuralization of platforms, we aim to examine how the commodification of life processes contest the feasibility of the government's "flexible employment" policy. Additionally, 
% the monetization process of daily life content on platforms, the disruptions of cultural production, and the cultivation of a new work and lifestyle under state governance in post-pandemic China.
%We ask the following research questions:
%\textbf{RQ1}: \textit{How Key Opinion Consumers are made in the social media platform marketing ?}
%\textbf{RQ2}: \textit{How do KOCs, marketers, and platform (?) coordinate and collaborate in the content creation process?}

\section{background}

% , including the use of mobile social networks and new media to expand social commerce and Internet marketing strategies.
% Entering the 2010s, the boosting Internet technologies and platform economy have been producing possibilities for new flexible employment. 
% penetrate different socio-economic sectors and update labor relations. In concurrent with the trend, in China, the younger generation of the working class, comprised of migrant peasant workers and those of lower degrees also joined it as drivers, delivery people, and task-based on-demand workers. 
% In the next section, we will trace and demonstrate how the Internet technologies and platform economy have updated flexible employment in China.
% In China, the state's intervention with the Internet technology and platform economy is ostensible. The Chinese state council, since 2015, has been promoting the ``Internet Plus Economy'' (互联网+经济\textit{hu lian wang jia jing ji}) \cite{guang2015}. This project is aimed at using Internet technologies to boost economic development in different sectors \cite{zhong2015}, including encouraging ``usage of mobile social networks and new media to develop social commerce (社交电商\textit{she jiao dian shang}) and other Internet marketing models'' \cite{zhong2015}.


\section{findings}

%-  platform arbitrage (in the assemblages)
%-  素人koc -- an informal influencer marketing strategy carried out by marketers and other brokers
%-  women's labor is integrated into the state's nation-building project

%- the emotional labor carried out by kocs - self-maintaining an ``authentic'' image, less intrusive product promotion, and "feeling good for myself"
%-  kocs update and create content to keep their middle-class-ness perpetuated by sensibilities for consumption 
%- xiaohongshu provides a legitimate place to promote products without considering how promotion ruin one's personal relations (cite zhang lin, p.213)

%Our research questions asked ..... We also asked.....

\subsection{5.1}

\subsubsection{5.1.1}

% \hy{Self-actualization was predicated on the feeling of being able to help others; also, Lexie thought the workplace experience was more beneficial to her followers after all, } especially those young professionals just like her.
% Reflecting on her experience following stylish content creators on Instagram who share chic daily outfits, she commented,} 
%Simply ``being good-looking'' or ``showing chic styles'' would not interest her followers for long. She gave the first author the example of an Instagram blogger she followed to elaborate, 
% \begin{quote}
% \textit{``I used to enjoy watching @vintageefeeling share daily styles in the beautiful scenery, but I lost interest finally. After all, it was helpless for me because I could not become as beautiful as they are after watching their postings and their content seemed repetitive.''}
% \end{quote}
% Lexie happily \hy{accepted her ``workplace content creator'' persona and }dedicated to posting about her workplace \hy{experiences}, thoughts, and reflections. , 


% \hy{When asked about her ultimate goal of posting on RED, Lexie didn't hesitate, ``Making money! (搞钱~\textit{gao qian}).'' Monetizing on RED, similar to any other social media platform, is highly relevant to the number of one account's followers. Having more followers promises potential visibility, which is often supported or thwarted by the platform's algorithmic design.} 
% %Working in the advertisement industry, Lexie knew basic influencer marketing strategies and some rules for engaging with her followers. The insider's knowledge promised Lexie the possibility to contest her content creation business on RED. 
% Towards the goal of making money, Lexie \hy{tactically looked into skills of gaining followers faster and came up with two rules of thumb.}
% %started with accumulating followers. Despite little expectation for the number of followers, the threshold of KOCs is 5,000 followers. Lexie concluded two strategies that were suitable for her. 
% First, she always used good-looking portrait photos as cover pictures for the postings to attract attention and clicks; second, she analyzed and caters to her followers’ needs and interests. \hy{For Lexie, ``good-looking'' meant being healthy and energetic.} \hy{Compared with the popular aesthetic on the Chinese Internet, which prefers pale skin and a skinny body, Lexie affirmed her perspective,} \textit{``Toned and tight muscular is more attractive.''} In Lexie’s cover portrait photos, she showed her arms and shoulders with toned lines gained from exercises; her sunshine-like smile seemed to indicate her persona, a healthy and energetic workplace smart, \hy{matching her professional image as a workplace content creator}. 


% In her opinion, \hy{inauthentic }social media \hy{content and certain aesthetic for women's appearance }generated anxiety \hy{for her}; sometimes, social media became the place for bragging about success or snooping into others’ private lives. But RED felt different for Shirley, \textit{``I found people on RED are more likely to `be oneself' and `not compare with others.' That’s why I like RED over other social media.''} \hy{Mundane content, encouraged by the platform's core value, differentiates RED from other social media platforms and captures users like Shirley, who is not a fan of social media.} 

% This insider knowledge equipped her to navigate and potentially advance her content creation business on RED. 

% \hy{Like Lexie, Shirley did not expect to gain hundreds of ``likes'' overnight on RED; instead, she used RED to record her daily life because of the boredom of working from home during COVID-19 in late 2020.} Her posting of Japanese restaurants in Dallas attracted attention, which \hy{positively motivated her} to use RED \hy{more}. \hy{Shirley found fun recording her daily life and interacting with her followers. Sharing daily life in Dallas and being a Dallas local guide comprises Shirley's persona on RED. To maintain this persona Shirley summarized her basic principle when creating content, that is} ``being oneself.'' \hy{In order to be} oneself, \hy{Shirley emphasizes the importance of} staying sincere and sharing useful experience to others, 
% \textit{``I believe that only `practical information (干货\textit{gan huo}) could be useful and beneficial to my followers and keep them with me.''}
% \hy{Reflecting on and connecting her own }experience of \hy{reading other's RED content, Shirley constantly thinks from her followers' perspective and makes sure her content is as useful. She pulled one example,} a female venture capital investor on RED to make her point, 
% \textit{``I enjoy reading something that really inspires or motivates me. Through reading her content, I learned how to become a businesswoman in this men-dominated world.''} 


% Her guiding principle for content creation is to ``be oneself.'' 
% Shirley that only thinking from her followers' perspectives can truly ensure her posts are helpful to her followers
% believes in the value of sincerity reflected in the content she shares through her posts. 
% Reflecting on her content consumption on RED, Shirley. Sirley recalls a female venture capital investor,  who was a content creator on RED whom she liked, inspired her own entrepreneurial ambitions,
% a content creator who label herself / have a persona of a female venture capital investor .... 
% \textit{``I enjoy reading something that really inspires or motivates me. Through reading her content, I learned how to become a businesswoman in this men-dominated world.''} 
% \hy{for her when she aspired to start her entrepreneurial projects}:
% \hy{Putting on the persona the platform curated for her, Shirley thought carefully about how to maintain her visibility and connection with other followers.} 
% she took inspiration from someone else's content --- to think about what she could do as a local guide / performing the persona

% Being a Dallas local guide content creator, Shirley ensured that her posts are genuinely helpful, especially for those Chinese living or sightseeing in the city. 
% Shirley enjoyed documenting her daily life on RED through her posts and interacting with her followers, 
%performing the persona of a local guide for Dallas on the platform. 

% \hy{who started their content creation work by accident, navigated the possibility of becoming a KOC through, first and foremost, performing the personas curated by the platform so as to 
% \hy{Being curated by the platform and enacting personas that they did not intend to present, content creators have to proactively align themselves with the personas the platform curated. Maintaining such personas structures content creators to put on a mindset and to pick up knowledge to play them out. It requires extra labor to understand what is preferred and what might be less effective, for both the platform and their audiences. However, the platform's visibility mechanism is often shrouded in ambiguity; in addition, the goal of monetizing their content creation by incorporating advertorials adds another layer of complexity to their labor. In the next section, we demonstrate their tactics for maintaining visibility while seeking monetization opportunities.} 


% This strategic approach to managing their visibility allowed them to effectively produce content for monetization. % advertorial
%Shirley's thoughts echoed Lexie's when it came to creating practical content. 

\subsubsection{5.1.2}

%\lx{Content creators on RED need to understand the needs of different stakeholders, including their followers and potential commercial partners, when selecting content topics and themes. 
%  In the following section, we explore their strategies for monetizing their content creation while maintaining visibility
% Meanwhile, creators need to match themselves with potential brands' needs and prepare themselves as if they are investable objects. 
% This section shows how content creators navigate the platform and please their followers and potential commercial collaborators.


%\hy{To assist content creators,} RED provided basic analytical data of their follower populations. 94\% of Lexie’s followers were women, 50\% were between age 18 and 24, 35\% were in Shanghai, and ``Education and Knowledge'' was the topic they were most interested in. Lexie \hy{categorized} her content with \hy{three} hashtags: ``fast-moving consumer goods industry knowledge,'' ``Fall campus recruitment interview Bible,'' and ``marketing in daily life.'' They each \hy{catered to a specific group of her followers}: the inside-industry knowledge for young professionals, job interview skills for new graduates, and fun facts for everyone. Lexie described \hy{the style of content} as ``tangible.''  She said, 
% \begin{quote}
%    \textit{Being tangible is concrete, not abstract. I hope people who read my posting can \hy{learn from my experience} and know how to do the interviews and perform better at work. I hope I am tangible, like a friend in my followers' life, not someone aloof.} 
% \end{quote}
% Being tangible, for Lexie, \hy{meant} to be practical, \hy{be close to the everyday life of every ordinary RED user}. 
% %In one of her most recent postings, Lexie shared three skills to make concise and clear slides for young professionals and students in college. In the comment area, her followers express their gratitude and compliment her, calling her content ``practical information'' (干货\textit{gan huo}). Despite unfriendly comments and doubts about Lexie’s content, she took them as a way to reflect on whether her content could indeed help people understand the fast-moving consumer goods industry. 


\subsection{5.2}

\subsubsection{5.2.1}

% The advertorial and her work experience content seamlessly merged into one video posting.
%\lx{她希望她的audience finds the content relatable, ... hope for an increase in her follower counts...}
%KOCs还要思考是否要生产同一种content。是的，因为要在这个领域中个看起来专业。增加credibility，增加influential power。
%整个事情的结果，是帮助KOC being vertical，帮助KOCs match到了更多的advertizers。
%\lx{In addition to fulfilling her audience's needs, being vertical also helps position Lexie for monetizing opportunities.} 

% As a workplace content creator, Lexie focused on work-related topics only. In her self-introduction on her RED account, \textit{``Do not create anxiety, produce substantial content, and grow with my followers.''} \hy{The practical information in a specific area that Lexie was dedicated to satisfied her followers' needs. In addition, her workplace professional persona and particular content themes made her appear to be ``vertical'' (垂直\textit{chui zhi}) in the workplace content creation area.} \hy{In such way, being vertical brings Lexie convenience when seeking monetizing opportunities. Once she reached the 10,000-follower threshold, Lexie was reached out by talent brokers--often known as multi-channel network (MCN) agencies in China. }

%\hy{Being vertical not only helps content creators like Lexie cater to the needs of her followers but also facilitates the potential to embed advertorials in their content so that they can monetize.}
%Shirley focused on four categories of topics: box-opening and product reviews, restaurant experience reviews in Dallas, travel and vacation tips, and personal reflections on general life experiences. Among all the topics, box-opening, and product reviews are the major ones where she inserted advertorial content, mostly facing Chinese living in Mainland China. When reviewing products, Shirley proudly claimed that she only spoke from her real experience and perceptions. This also contributes to what she meant by ``being oneself'' -- that is to stay true. The responsible attitude toward her content does not dismiss the difficulty in actual practices. Since she spent a large amount of time in Dallas, the product mailing became rather tricky. The products popular in China might not be available in the USA. Such an issue prevented Shirley from producing more product-review content, and, at the same time, refrained her from being ``vertical.'' Shirley complained that her account feed appeared to be diverse with all kinds of content, but she had a hard time categorizing herself into the expert in none of the four main topics she positioned in. Being slightly deviated from cultivating her verticality in one topic frustrated Shirley and hindered her from scaling up. Shirley framed her anxiety as a question and posted it to the first author during the interview in the hope of brainstorming and advice. 
% 其实我觉得这个细节挺好的，resources that Shirley can get access to as a person influences her content production ----- 这个是informal labor的一个侧面，没有institutional / organizational support, creators need to figure out their own ways

% The preference for a large number of KOCs is shaped by the impenetrable platform algorithm that curates content.
%\hy{Given KOCs' limited influencing power, marketers' expected monetary rewards for each KOC is very little, or even none sometimes.}  %With the same amount of budget, marketers can purchase and collaborate with many more KOCs whose content can reach more RED users’ feeds. 
%KOC's personas help to consumers to be persuaded into purchasing the products.} 
%so that they may be more likely to be convinced by the advertisements. 
%The less embellished content appears to be more relatable and inspiring.
%as a way for ordinary platform users to form further interactions and discussions. 
%``Tap water'' \hy{echos the sociological concept of} prosumers \cite{Toffler} \major{who produce} new digital content, \major{voicing} for the brands and products for free, as they consume \hy{the digital content} on the platform.

%Celia worked as an international indie skincare brand, in charge of social media placement (which refers to the process of choosing channels for advertisement \cite{noauthor_what_nodate}).
%https://www.verticalimpression.com/post/what-is-digital-media-placement-and-5-steps-to-build-a-successful-media-placement-strategy
%The number of KOCs her campaigns featured ranged from tens to hundreds. We have presented that marketers expect to ``cast a wide net'' and involve as many KOCs in each campaign as the budget allows. %The appearance of countless ordinary users on the RED platform talking about one product or brand create the impression that the product is popular. 

%However, going through pages of Excel and securing a certain number of content creators is a task subordinate to making the decision of which KOC is a fit and which is not. 
%appears to be judgmental or even acerbic in that the popularity of one content creation relies highly on 
%The marketers’ job, at this stage, is to go through the spreadsheet and \hy{decide whom they want to collaborate with}. The physical labor performed by marketers is infrastructural to building a given brand’s own ``KOC talent pool,'' while the process of finding as many KOCs who are fit for the campaign as possible is time-consuming work. According to Celia,
%\begin{quote}
%   \textit{I manually go through the Excel spreadsheets. I go to the potential KOCs’ \hy{personal} account profiles and \hy{investigate all the} content \hy{they have created }in the past…it’s \hy{pure} manual work… thousands of them.}
%\end{quote}

% The KOC has to be dedicated to one particular area; I judge them by looking into their account profile. If this KOC has all kinds of content, for example, they have content in skincare, makeup, baby care, food, and vacation… they are not vertical, and .
%The ``indie'' trait that the indie brand that Celia worked for wanted to address differentiated the brand’s communication messages from the others. The brand focused on the ``ingredients'' and “efficacy” of the products. 
The preference for verticality echoes content creators like Lexie's and Jasper's tactics of producing niche content. However, in marketer's eyes, too much verticality is neither an expected trait. Celia commented, 
%Celia composed and edited general communication brief messages and disseminated the documents through social media advertisement agencies to KOCs. This brief message is constructed to help KOCs to sound like experts. However, Celia comments, \textit{``If KOCs only use the brief message, it will be too explicit.''} 
\hy{After all, KOCs are everyday platform users,} the content they create should be mundane and less intrusive, even if it is advertisement-oriented. KOCs are expected to speak consumers' minds, appearing to be like every other RED user. \hy{With such a specific requirement, marketers would go through and check every word in KOC's posting.}\hy{For the content creators, these specific expectations are not transparent to them; instead, they need to figure it out as they go forth and back, re-editing their content after receiving rounds of feedback from marketers. Once their content is accepted by marketers, content creators can eventually gain some monetary rewards.}
%Being persuasive with expertise does not mean that KOCs have to tell the boring scientific mechanism \hy{behind} products; 

%In addition, effective interactions with followers are an index for Celia to make the judgment of whether the KOC is ideal for her brand. Again, whether a KOC is too explicit in their advertorial content or interacts well with their followers is judged by marketers’ perception.

\subsubsection{5.2.2}

%As individual marketers rely on their sensibilities to select fit KOLs/KOCs, the companies, emphasizing return on investment (ROI) stabilize the KOL/KOC selection procedures via internal bureaucratic work. Celia describes how she initiated, reported, and finalized the KOC procurement according to the corporation's organizational requirements. 

%\begin{quote} \textit{For each campaign, I have to go to the corporation’s internal KOL/KOC procurement system. I input the number of KOLs/KOCs I need and my rough budget for RED placement to initiate the price comparison. Once the procurement department sees my request, they will go through my request and give me the approval, or reject me. They will then invite all social agencies the corporation co-works within the market to provide their quotations. The agencies will then reach out to KOLs/KOCs through the Multi-Channel Networks (MCN) agencies. Note that the commissions for each MCN may vary. The social agency with the lowest bidding price will be the winner.}
%\end{quote}

%The internal procedure is more than just bureaucratic work; rather, it reflects an underlying standard for the business organization to decide what makes a good KOL/KOC. 

%One critical index the procurement department looks for, before granting the approval, is the ratio between the number of ``like'' and the follower number one particular KOL/KOC has. It is termed as ``cost per real engagement'' (CPRE) in Celia’s company. \footnote{``Real engagement'' means effective engagement where the followers interact with the content creators by commenting with meaning or staying on the page longer than a certain number of seconds.} The organizational internal interpretation of high CPRE indicates high follower ``stickiness.'' Customer stickiness refers to the ability of a product or service to retain customers over an extended period \cite{stickiness}, and the concept is particularly popular in the tech industry when assessing a digital product. Applying and adjusting the concept to measure a KOC, a human content creator, transforms a human into a measurable object.   

%Different companies use different measures to quantify the performances and effectiveness of KOLs/KOCs on RED. For example, marketer Kathy's company, another multinational company investing heavily in marketing in Shanghai, uses cost per engagement (CPE) to measure each content posting’s performance. CPE is the ratio between the cost of one particular KOL/KOC posting and the ``like'' number it gains. Different from CPRE, CPE measures the monetary cost of each digital content on RED, considering the immediate investment returns more than long-term rewards brought by loyal customers. Both CPRE and CPE, in a quantifiable way, entail how a KOC’s value can be measured and calculated. They provide accountability to marketers and transfer a seemingly subjective and volatile process of selecting KOCs into an organizational procedure. 

%Interestingly still, according to both Celia and Kathy, this well-designed quantitative measurement was more commonly used with KOL procurement. When it came to KOCs, the complexity of going through the bureaucratic work prevented marketers and the procurement department from walking the KOCs through the corporation system. This leaves the KOCs out of the consideration of the corporation; further, it pushes the decision-making process to marketers who can only rely on their personal perception and experience. C In the marketing practices that address the reward of investment, KOCs' value remains unclear and even invisible to the management system.

In this part, we elaborate on the corporations' internal working procedures, in which the marketers' are involved. As marketers select fit content creators and make them KOCs in campaigns on RED, at the organizational level, especially the clerical work, the KOCs are invisible. We show how KOCs and their labor are invisiblized from the corporation's clerical systems.

Before each campaign, marketers have to go through the procurement procedure to apply for a budget, which is used to pay KOCs, as well as KOLs and celebrities, and the RED platform. Marketers have to report the itemized budget plans to the procurement department. The latter invited different social agencies to tender for service contracts. The social agencies with the lowest bidding price win. Usually, itemized budget plans require marketers to provide several sets of data to measure the return on investment. The corporation looks for the ratio between the number of ``likes'' and the follower number one particular content creator has. It is termed CPRE (cost per real engagement)~\footnote{``Real engagement'' means effective engagement where the followers interact with the content creators by commenting with meaning or staying on the page longer than a certain number of seconds.}. From the corporation's perspective, the higher CPRE indicates that the content creators' followers are ``stickier.'' It means that the content creators have the ability to retain their followers over an extended period \cite{stickiness}. \footnote{``Stickiness'' concept is particularly popular in the tech industry when assessing a digital product.} In addition, CPE (cost per engagement), the ratio between the cost of one particular content creator's posting and the ``like'' number it gains, is also required to measure the immediate investment returns content creators can bring. The itemized budget plans and the measurable indexes help to stabilize the RED platform influencer marketing working processes. Such stabilization is critical to guarantee each stakeholder's benefits.

However, the KOCs are excluded from the itemized budget plans. To avoid complicated clerical work, in actual practice, the budgets intended for KOC payment are distributed and located in those for KOLs or celebrities. Celia commented, \textit{``Because KOCs cost only little money.''} In other words, it is not worthwhile going through the excessive paperwork for KOCs. In this way, KOCs become invisible, hiding in the backstage of marketing campaigns. Ironically, involving KOCs in RED campaigns is a widely used business strategy in the advertising industry. The invisibility of KOCs from corporation clerical work and stabilized working processes brings KOCs precarity; in that the rewards of their content creation are dependent on informal agreement in the triangular relationship among KOCs, the corporation, and the RED platform. In the next part, we turn to the RED platform and show how the platform further invisiblizes KOCs from the stabilized working processes. 

\subsubsection{5.2.3}

%For the RED platform, KOCs are out of the RED’s concerns. Before we unpack how KOCs are free from the platforms' regulation, we describe how the platform surveils the KOLs, who have more followers, in the marketing campaign. In the marketing campaigns with KOLs, brands are required to report (报备\textit{bao bei}) their advertorial content to the platform through RED’s embedded ``Deadilon'' (蒲公英\textit{pu gong ying}) platform. The marketers are told by the representatives of the RED platforms, that reporting is beneficial to brand marketers. Usually, according to Celia, the business developing team of the RED platform would come in contact with brand marketers. Once the advertisement is reported, the platform's curating system would not be limited; and the digital content would be exposed to the platform users as much as possible. The consequences of not reporting KOL campaigns and advertisements to Deadilon, for brands, are severe. Celia gives several examples of both Chinese domestic and international brands that she has witnessed. They are banned from RED’s search engine for a certain period (usually at least 10 days), which is detrimental to the brands’ exposure and impacts in the market that changes fast. The reporting requirement is described by the platform representatives as helpful in managing the ratio of advertorial content and content from real ordinary users. 
%In contrast, the KOCs seem to have more freedom to create advertorial content in collaboration with brands. Collaboration between brands and KOCs is not part of the RED platform's reporting requirement. Such a lack of regulations on KOCs reflects the platform's perspective: KOCs are more ordinary users than content creators in advertorial processes. On the one hand, it allows marketers the opportunity to develop a KOC-oriented marketing strategy. On the other hand, it puts KOCs in an underestimated position, from which they and their content creation can be devalued or even dismissed because they are less likely to be considered valuable as a piece of advertorial content. In reality, to make their content count, individual KOCs put much effort into making themselves and their content valuable. In the following, we unpack how KOCs, as individual laborers, perform cultural and creative labor to create content for advertorial purposes. Their work is relational in a chain of labor taken upon by multiple actors in the marketing industry. 
%Then, we show how platforms make use of the labor of multiple stakeholders to build cultural values which are core to configurate its technological design and business mechanism.
%\subsection{Making Key Opinion Consumers in Practices}
%\subsubsection{Quantified Measurement}
%As individual marketers rely on their sensibilities to select fit KOLs/KOCs, the companies, emphasizing return on investment (ROI) stabilize the KOL/KOC selection procedures via internal bureaucratic work. Celia describes how she initiated, reported, and finalized the KOC procurement according to the corporation's organizational requirements. 
%\begin{quote}
%\textit{For each campaign, I have to go to the corporation’s internal KOL/KOC procurement system. I input the number of KOLs/KOCs I need and my rough budget for RED placement to initiate the price comparison. Once the procurement department sees my request, they will go through my request and give me the approval, or reject me. They will then invite all social agencies the corporation co-works with in the market to provide their quotations. The agencies will then reach out to KOLs/KOCs through the Multi-Channel Networks (MCN) agencies. Note that the commissions for each MCN may vary. The social agency with the lowest bidding price will be the winner.}
%\end{quote}
%The internal procedure is more than just bureaucratic work; rather, it reflects an underlying standard for the business organization to decide what makes a good KOL/KOC. One critical index the procurement department looks for, before granting the approval, is the ratio between the number of ``like'' and the follower number one particular KOL/KOC has. It is termed as ``cost per real engagement (CPRE)'' in Celia’s company. \footnote{``Real engagement'' means effective engagement where the followers interact with the content creators by commenting with a meaning or stay on the page longer than certain number of seconds.} The organizational internal interpretation of high CPRE indicates high follower ``stickiness.'' Customer stickiness refers to the ability of a product or service to retain customers over an extended period \cite{stickiness}, and the concept it particular popular in tech industry when assessing a digital product. Applying and adjusting the concept to measure a KOC, a human content creator, transforms a human into a measurable object.  
%Different companies use different measures to quantify the performances and effectiveness of KOLs/KOCs on RED. For example, marketer Kathy's company, another multinational company investing heavily in marketing in Shanghai, uses cost per engagement (CPE) to measure each content posting’s performance. CPE is the ratio between the cost of one particular KOL/KOC posting and the ``like'' number it gains. Different from CPRE, CPE measures the monetary cost of each digital content on RED, considering the immediate investment returns more than long-term rewards brought by loyal customers. Both CPRE and CPE, in a quantifiable way, entail how a KOC’s value can be measured and calculated. They provide accountability to marketers and transfer a seemingly subjective and volatile process of selecting KOCs into an organizational procedure. 
%Interestingly still, according both Celia and Kathy, this well-designed quantitative measurement was more commonly used with KOL procurement. When it came to KOCs, the complexity of going through the bureaucratic work prevented marketers and procurement department from walking the KOCs through the corporation system. This leaves the KOCs out of the consideration of the corporation; further, it pushes the decision-making process to marketers who can only rely on their personal perception and experience. Celia commented, \textit{``Because KOCs cost only little money.''{KOCs' value remains unclear and even invisible to the management system in the marketing practices that address the reward of investment.}


\subsection{5.3}

\subsubsection{5.3.1}

While Shirley experimented with other potential topics she could shift to and found her followers tending to send more likes to her box-opening and product review videos. 
However, most of her followers are Chinese in Mainland China while she spent a large amount of time in Dallas. The product mailing became tricky when making product-review videos since products popular in China might not be available in the US. Such an issue worried Shirley and almost forced her to try other topics. Shirley complained that her account feed appeared to be messy and had a hard time establishing her verticality in one area, which would impact her ability to keep her followers engaged. For both Jasper and Shirley, because of the ad-hoc nature of advertorial collaboration with marketing campaigns, they are worried that they cannot monetize anymore if they lose their followers.

For both Jasper and Shirley, because of the ad-hoc nature of advertorial collaboration with marketing campaigns, they are worried that they cannot monetize anymore if they lose their followers.

\subsubsection{5.3.2}




